Magnetohydrodynamic structure of a plasmoid in fast reconnection in low-beta plasmas

Plasmoid structures in fast reconnection in low-beta plasmas are investigated by two-dimensional magnetohydrodynamic simulations. A high-resolution shock-capturing code enables us to explore a variety of shock structures: vertical slow shocks behind the plasmoid, another slow shocks in the outer-region, and the shock-reflection in the front side. The Kelvin-Helmholtz-like turbulence is also found inside the plasmoid. It is concluded that these shocks are rigorous features in reconnection in low-beta plasmas, where the reconnection jet speed or the upstream Alfven speed exceeds the sound speed.

==> Ancillary_files_20110112/1D/Makefile <==
F90 = /opt/intel/Compiler/11.1/067/bin/intel64/ifort
#F90 = gfortran -O2 -m64 -Wall

OBJS = model.o set_dt.o u2v.o output.o \
	v2u.o v2f.o v2g.o limiter_f.o limiter_g.o \
	hlld_f.o hlld_g.o hllc_f.o hllc_g.o hll_f.o hll_g.o llf_f.o llf_g.o

all: 1d_x 1d_y
	./1d_x && ./1d_y

1d_x : 1d_x.o $(OBJS)
	$(F90) -o 1d_x 1d_x.o $(OBJS)

1d_y : 1d_y.o $(OBJS)
	$(F90) -o 1d_y 1d_y.o $(OBJS)

%.o: %.f90 $(MODULES)
	$(F90) $(FFLAGS) -c $<

clean :
	rm -f 1d_x 1d_y *.o data/*.dat


==> Ancillary_files_20110112/2D/Makefile <==
#F90 = /opt/intel/Compiler/11.1/067/bin/intel64/ifort
F90 = gfortran -O2 -m64 -Wall

OBJS = model.o set_dt.o u2v.o output.o rk21.o rk22.o step1.o step2.o bc.o \
	v2u.o v2f.o v2g.o limiter_f.o limiter_g.o \
	hlld_f.o hlld_g.o hllc_f.o hllc_g.o hll_f.o hll_g.o llf_f.o llf_g.o \
	glm_f.o glm_g.o glm_ss.o

run : main.o $(OBJS)
	$(F90) -o a.out main.o $(OBJS)

%.o: %.f90 $(MODULES)
	$(F90) $(FFLAGS) -c $<

clean :
	rm -f a.out *.o data/*.dat


==> Ancillary_files_20110112/KH/Makefile <==
#F90 = /opt/intel/Compiler/11.1/067/bin/intel64/ifort
F90 = gfortran -O2 -m64 -Wall
F90 = /opt/openmpi64g/bin/mpif90 -Wall

OBJS = model.o set_dt.o u2v.o output.o rk21.o rk22.o step1.o step2.o bc.o \
	v2u.o v2f.o v2g.o limiter_f.o limiter_g.o bc_fixv_g.o \
	hlld_f.o hlld_g.o hllc_f.o hllc_g.o hll_f.o hll_g.o llf_f.o llf_g.o \
	glm_f.o glm_g.o glm_ss.o
OBJP = modelp.o mpibc.o mpi_fixv_f.o

all: run runp

run : main.o $(OBJS)
	$(F90) -o a.out main.o $(OBJS)

runp : mainp.o $(OBJS) $(OBJP)
	$(F90) -o ap.out mainp.o $(OBJS) $(OBJP)

%.o: %.f90 $(MODULES)
	$(F90) $(FFLAGS) -c $<

clean :
	rm -f *.out *.o data/*.dat


==> Ancillary_files_20110112/RX/Makefile <==
#F90 = /opt/intel/Compiler/11.1/067/bin/intel64/ifort
F90 = gfortran -O2 -m64 -Wall
F90 = /opt/openmpi64g/bin/mpif90 -Wall
F90 = mpif90 -O2 -m64 -Wall

OBJS = model.o set_dt.o set_dt2.o set_eta.o u2v.o output.o rk21.o rk22.o step1.o step2.o bc.o \
	v2u.o v2f.o v2g.o limiter_f.o limiter_g.o bc_fixv_g.o \
	hll_resistive_f.o hll_resistive_g.o glm_f.o glm_g.o glm_ss.o
OBJP = modelp.o  mpibc.o  mpi_fixv_f.o
OBJP2= modelp2.o mpibc2.o mpi_fixv_f2.o bc_fixv_g2.o

all: run runp runp2

# serial version
run : main.o $(OBJS)
	$(F90) -o a.out main.o $(OBJS)

# parallel version
runp : mainp.o $(OBJS) $(OBJP)
	$(F90) -o ap.out mainp.o $(OBJS) $(OBJP)

# parallel version (1/4 BC for large-scale evolution)
runp2 : mainp2.o $(OBJS) $(OBJP2)
	$(F90) -o ap2.out mainp2.o $(OBJS) $(OBJP2)

%.o: %.f90 $(MODULES)
	$(F90) $(FFLAGS) -c $<

clean :
	rm -f *.out *.o data/*.dat

